E$^2$(GO)MOTION: Motion Augmented Event Stream for Egocentric Action Recognition

Event cameras are novel bio-inspired sensors, which asynchronously capture pixel-level intensity changes in the form of "events". Due to their sensing mechanism, event cameras have little to no motion blur, a very high temporal resolution and require significantly less power and memory than traditional frame-based cameras. These characteristics make them a perfect fit to several real-world applications such as egocentric action recognition on wearable devices, where fast camera motion and limited power challenge traditional vision sensors. However, the ever-growing field of event-based vision has, to date, overlooked the potential of event cameras in such applications. In this paper, we show that event data is a very valuable modality for egocentric action recognition. To do so, we introduce N-EPIC-Kitchens, the first event-based camera extension of the large-scale EPIC-Kitchens dataset. In this context, we propose two strategies: (i) directly processing event-camera data with traditional video-processing architectures (E$^2$(GO)) and (ii) using event-data to distill optical flow information (E$^2$(GO)MO). On our proposed benchmark, we show that event data provides a comparable performance to RGB and optical flow, yet without any additional flow computation at deploy time, and an improved performance of up to 4% with respect to RGB only information.

==> Tab/Fusion.tex <==
\begin{table*}[h]
\begin{minipage}{\linewidth}
\begin{adjustbox}{width=0.7\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{ccc|cc|cc}
\toprule\noalign{\smallskip}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Late fusion}} & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{\textbf{TRN}} \\ \cline{2-7} \noalign{\smallskip}
                & \textbf{S-Acc (\%)}           & \textbf{U-Acc (\%)}          & \textbf{S-Acc (\%)}       & \textbf{U-Acc (\%)}      & \textbf{S-Acc (\%)}      & \textbf{U-Acc (\%)}      \\ \hline\noalign{\smallskip}
TSM                  &    64.38	 & 37.75 & 63.75       & 36.46      & 63.65      & 37.28      \\ \hline\noalign{\smallskip}
TSN                  &                 &                &             &            &            &            \\ \hline\noalign{\smallskip}
I3D                  & 55.54 &	37.52         & 53.64       & 36.59      & 55.88      & 36.37  \\
\bottomrule\noalign{\smallskip}

\end{tabular}
\end{adjustbox}
\end{minipage}
\caption{supp}
\label{tab:fusion}

\end{table*}


==> Tab/Mars.tex <==

\begin{table*}[]
\begin{minipage}{\linewidth}
\begin{adjustbox}{width=0.5\columnwidth, margin=0ex 1ex 0ex 0ex}

\begin{tabular}{lllccc}
\toprule\noalign{\smallskip}
%\begin{table}[t]
%\begin{tabular}{lllccc}

Stream  & Model  & $\lambda$ & \multicolumn{1}{l}{Seen} & \multicolumn{1}{l}{Unseen} \\ \hline
RGB  & TSM     & &    71.48	 &  35.97         \\
RGB + distil   & TSM   & 50 &                       72.77 &	39.36      \\
RGB + distil  & TSM   & 100 &       Update             &    \textbf{Update}       \\\hline
Event           & Vox-TSM       &  &    65.40                &   	40.33              \\ 
Event + distil      & Vox-TSM           & 50 &    69.43		   &    44.40 \\ 
Event + distil      & Vox-TSM           & 100 &    70.76		   &    \textbf{45.57} 
\\ \hline



\end{tabular}
\end{adjustbox}
\caption{placeholder}

\end{minipage}



\end{table*}


==> Tab/MultiModal.tex <==

\begin{table}[]
\begin{adjustbox}{width=\columnwidth, margin=0ex 1ex 0ex 0ex}
\begin{tabular}{lllccc}
\toprule\noalign{\smallskip}
\textbf{Stream}         & \textbf{Model}   & \multicolumn{1}{l}{\textbf{Seen}} & \multicolumn{1}{l}{\textbf{Unseen}} \\ \hline\noalign{\smallskip}




Event+Flow (PWC-Net)      & I3D   &     61.58 &	{43.52}                           \\ 
Event+Flow (TV-L1)      & I3D   &    \textbf{62.66}   &                    \textbf{45.86}        \\ \hline
RGB+Flow (PWC-Net)      & I3D   &     58.90 &	40.68  \\ 
RGB+Flow (TV-L1)      & I3D   &   62.07             &                      44.56   \\ \hline
RGB+Event    & I3D     &  61.23 &                    41.85  \\ 

\hline\hline


Event+Flow (PWC-Net)      & TSM          &   Update                         &                     Update   \\ 
Event+Flow (TV-L1)      & TSM    &   Update	& \textbf{Update}          \\ 
\hline
RGB+Flow (PWC-Net)      & TSM    &    Update                        &                       Update    \\ 
RGB+Flow (TV-L1)      & TSM   & Update              &                      Update   \\ \hline
RGB+Event    & TSM   &  71.88	           &                   39.92 \\ 


\bottomrule
\end{tabular}
\end{adjustbox}
\caption{supp}

\end{table}

==> Tab/Ours.tex <==
\begin{table*}[]
\begin{tabular}{ll|rrr|rrrrrr|cc}
\toprule\noalign{\smallskip}

         Method & Model & \multicolumn{1}{c}{\textbf{D1}} & \multicolumn{1}{c}{\textbf{D2}} & \multicolumn{1}{c|}{\textbf{D3}} & \multicolumn{1}{c}{\textbf{D1-D2}} & \multicolumn{1}{c}{\textbf{D1-D3}} & \multicolumn{1}{c}{\textbf{D2-D1}} & \multicolumn{1}{c}{\textbf{D2-D3}} & \multicolumn{1}{c}{\textbf{D3-D1}} & \multicolumn{1}{c|}{\textbf{D3-D2}} & \multicolumn{1}{l}{\textbf{Seen}} & \multicolumn{1}{l}{\textbf{Unseen}} \\ \cline{0-12} \noalign{\smallskip}
Baseline& TSM & 55.61                  & 68.09                  & 66.40                   & 28.86                                    & 33.64                                    & 35.58                                    & 39.67                                    & 39.23                                    & 43.50                                     & 63.37                          & 36.75                          \\ \noalign{\smallskip}
Dist &TSM&     57.64                  & 69.30                  & 66.89                   & 34.47                                    & 35.52                                    & 38.74                                    & 43.28                                    & 37.87                                    & 46.60                                     & 64.61                          & 39.41                          \\ \noalign{\smallskip}
SS  &TSM&      56.61                  & 68.47                  & 66.81                   & 33.07                                    & 31.21                                    & 41.03                                    & 45.61                                    & 40.98                                    & 48.53                                     & 63.96                          & 40.07                          \\ \noalign{\smallskip}
SS+Dist  &TSM& 57.99                  & 69.17                  & 68.53                   & 34.47                                    & 33.80                                    & 44.25                                    & 45.23                                    & 41.95                                    & 52.37                                     & \textbf{65.23}                 & \textbf{42.01}     \\
    \bottomrule

\end{tabular}

\caption{Placeholder}
\end{table*}



==> Tab/channels.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{cclcc}
\toprule\noalign{\smallskip}
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{l}{\textbf{Voxel ch.}} & \textbf{Testing} & \multicolumn{1}{l}{\textbf{Seen acc}} & \multicolumn{1}{l}{\textbf{Unseen acc }} \\ \hline
\multirow{6}{*}{I3D}       & \multirow{2}{*}{9}                & Clip    & 49.84                          & 34.52                         \\
                           &                                   & Video   & \textbf{52.50}                 & \textbf{36.24}                \\ \cline{2-5} 
                           & \multirow{2}{*}{3}                & Clip    & 53.75                          & 35.90                         \\
                           &                                   & Video   & \textbf{55.54}                 & \textbf{37.52}                \\ \cline{2-5} 
                           & \multirow{2}{*}{1}                & Clip    & 49.34                          & 34.93                         \\
                           &                                   & Video   & \textbf{51.29}                 & \textbf{35.05}                \\ \hline
\multirow{6}{*}{TSN}       & \multirow{2}{*}{9}                & Clip    & 57.28&	31.74  \\
                           &                                   & Video   & \textbf{58.98} &	\textbf{32.52}          \\ \cline{2-5} 
                           & \multirow{2}{*}{3}                & Clip    & 58.81 &	34.65                         \\
                           &                                   & Video   & \textbf{59.82} &	\textbf{35.24}                \\ \cline{2-5} 
                           & \multirow{2}{*}{1}                & Clip    &	  52.59      &   30.94         \\
                           &                                   & Video   & \textbf{54.54}	        & \textbf{31.87}          \\ \hline
\multirow{6}{*}{TSM}       & \multirow{2}{*}{9}                & Clip    & 65.02	 &	37.65 \\
                           &                                   & Video   & \textbf{66.39}	 &	\textbf{38.71}       \\ \cline{2-5} 
                           & \multirow{2}{*}{3}                & Clip    & 64.38               & 37.75               \\
                           &                                   & Video   & \textbf{65.93}                         & \textbf{38.23}                         \\ \cline{2-5} 
                           & \multirow{2}{*}{1}                & Clip    & 60.76	& 34.66                        \\
                           &                                   & Video   & \textbf{62.46} &	\textbf{36.45 }           \\ 
                           \bottomrule

\end{tabular}
\caption{Placeholder}\label{tab:channels_}
\end{table}
